Mask CTC: Non-Autoregressive End-to-End ASR with CTC and Mask Predict

We present Mask CTC, a novel non-autoregressive end-to-end automatic speech recognition (ASR) framework, which generates a sequence by refining outputs of the connectionist temporal classification (CTC). Neural sequence-to-sequence models are usually \textit{autoregressive}: each output token is generated by conditioning on previously generated tokens, at the cost of requiring as many iterations as the output length. On the other hand, non-autoregressive models can simultaneously generate tokens within a constant number of iterations, which results in significant inference time reduction and better suits end-to-end ASR model for real-world scenarios. In this work, Mask CTC model is trained using a Transformer encoder-decoder with joint training of mask prediction and CTC. During inference, the target sequence is initialized with the greedy CTC outputs and low-confidence tokens are masked based on the CTC probabilities. Based on the conditional dependence between output tokens, these masked low-confidence tokens are then predicted conditioning on the high-confidence tokens. Experimental results on different speech recognition tasks show that Mask CTC outperforms the standard CTC model (e.g., 17.9% -> 12.1% WER on WSJ) and approaches the autoregressive model, requiring much less inference time using CPUs (0.07 RTF in Python implementation). All of our codes will be publicly available.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> subtex/_02_nar_asr.tex <==
\section{Non-autoregressive speech recognition}
The objective of end-to-end ASR modeling is to model the joint probability of a $L$-length output sequence $Y = \{ y_l \in \mathcal{V} | l=1,...,L \}$ given a $T$-length input sequence $X = \{\bm{\mathrm{x}}_t \in \mathbb{R}^D| t=1,...,T\}$. Here, $y_l$ is an output token at position $l$ in the vocabulary $\mathcal{V}$ and $\bm{\mathrm{x}}_t$ is $D$-dimensional acoustic feature at frame $t$.

The following subsections first explain an conventional autoregressive framework based on CTC and attention-based encoder-decoder.
% jointly trains an attention-based encoder-decoder model with CTC objective.
Then a non-autoregressive ASR model trained with mask prediction is explained and, finally, the  proposed non-autoregressive decoding method is introduced.

\subsection{Joint CTC-attention Autoregressive ASR}
To achieve robust alignment training and fast convergence, 
an end-to-end ASR model based on an attention-based encoder-decoder framework is trained with CTC~\cite{kim2017joint, karita2019improving}.

Attention-based encoder-decoder models the joint probability of $Y$ given $X$ by factorizing the probability based on the probabilistic left-to-right chain rule as follows:
\begin{equation}
    \label{eq:p_att}
     P_{\mathrm{att}} (Y | X) = \prod_{l=1}^{L} P_{\mathrm{att}} (y_l | y_{<l}, X).
\end{equation}
The model estimates the output token $y_l$ at each time-step conditioning on previously generated tokens $y_{<l}$ in an autoregressive manner. 
In general, during training, 
the ground truth tokens are used for the history tokens $y_{<l}$ and 
during inference, the predicted tokens are used.

CTC predicts a frame-level alignment between the input sequence $X$ and the output sequence $Y$ by introducing a special \texttt{<blank>} token and a special function $\beta$ which takes the frame-level alignment as an input and outputs the token-level sequence.
The alignment $A=\{ a_t \in \mathcal{V} \cup \{\texttt{<blank>}\} | t=1,...,T\}$ is predicted with the conditional independence assumption between the output tokens as follows:
\begin{equation}
    P_{\mathrm{ctc}} (A | X) = \prod_{t=1}^{T} P_{\mathrm{ctc}} (a_t | X).
\end{equation}
Considering the probability distribution over all possible alignments, 
CTC models the joint probability of $Y$ given $X$ as follows:
\begin{equation}
    \label{eq:p_ctc}
    P_{\mathrm{ctc}} (Y | X) = \sum_{A \in \beta^{-1} (Y)} P_{\mathrm{ctc}} (A | X),
\end{equation}
where $\beta^{-1} (Y)$ returns all possible alignments compatible with $Y$.
Regarding the computational cost for calculating the probabilities for all of the alignments, 
$P_{\mathrm{CTC}}(Y | X)$ can be computed efficiently using dynamic programming.

The objective of the autoregressive joint CTC-attention model is defined as follows using the formulations from Eq. (\ref{eq:p_att}) and Eq. (\ref{eq:p_ctc}):
\begin{equation}
    \label{eq:ctc-att}
    \mathcal{L}_{\mathrm{AR}} = \lambda \log P_{\mathrm{ctc}} (Y | X) + 
    (1 - \lambda) \log P_{\mathrm{att}} (Y | X), 
\end{equation}
where $\lambda$ is a tunable parameter.

\subsection{Mask-based non-autoregressive ASR}
Trained to predict mask tokens \texttt{<MASK>} in the target sequence~\cite{devlin2019bert}, 
conditional masked language model (CMLM)~\cite{ghazvininejad2019mask} is adopted for non-autoregressive speech recognition~\cite{chen2019non}.
Note that CMLM is applied to the training of the decoder, 
not external language model often used in shallow fusion during decoding.
Taking advantages of Transformer's parallel computation~\cite{vaswani2017attention}, 
CMLM can predict any arbitrary subset of masked tokens in the target sequence by attending to the entire sequence.

CMLM predicts a set of masked tokens $Y_{\mathrm{mask}}$ conditioning on the input sequence $X$ and part of the target tokens $Y_{\mathrm{obs}}$ as follows:
\begin{equation}
      P_{\mathrm{cmlm}} (Y_{\mathrm{mask}} | Y_{\mathrm{obs}}, X) = 
      \prod_{y \in Y_{\mathrm{mask}}} P_{\mathrm{cmlm}} (y | Y_{\mathrm{obs}}, X),
      \label{eq:p_cmlm}
\end{equation}
where $Y_{\mathrm{obs}}  = Y \setminus Y_{\mathrm{mask}}$.
During training, 
the ground truth tokens are randomly replaced with a special \texttt{<MASK>} token and CMLM is trained to predict the original tokens conditioning on the input sequence and the unmasked tokens.
The number of tokens to be masked is sampled from a uniform distribution between 1 to $L$ as in~\cite{ghazvininejad2019mask}.
During inference, 
the target sequence is gradually generated in a constant number of iterations $K$ by the mask-predict algorithm~\cite{ghazvininejad2019mask} 
which repeatedly masks and predicts the subset of the target sequence.
% Decoding starts with completely masked target tokens with a predicted legnth and 
% the model replaces the masked tokens with the predicted ones with high-confidence.
% The model then predicts the difficult masked tokens based on the previous high-confident tokens. 
% The target sequence is finally generated via this m
% The number of masks to be predicted at decoding iteration $k$ can be defined by using linear decay 
% $L \cdot \frac{K - k}{K} $, 
% where $K$ is the total number of iterations.

We observed that applying the original CMLM to non-autoregressive speech recognition shows poor performance, having the problem of skipping and repeating of the output tokens.
To deal with this, 
we found that jointly training with CTC provides the model with absolute positional information (conditional independence) explicitly and improves the model performance reasonably well.
With the CTC objective from Eq. (\ref{eq:p_ctc}) and Eq. (\ref{eq:p_cmlm}), the objective of joint CTC-CMLM training for non-autoregressive ASR model is defined as follows:
\begin{dmath}
    \label{eq:ctc-cmlm}
    \mathcal{L}_{\mathrm{NAR}} = 
    \gamma \log P_{\mathrm{ctc}} (Y | X) + 
    (1 - \gamma) \log P_{\mathrm{cmlm}} (Y_{\mathrm{mask}} | Y_{\mathrm{obs}}, X),
\end{dmath}
where $\gamma$ is a tunable parameter.

\subsection{Proposed decoding using CTC outputs}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6 \columnwidth]{img/figure.png}
    \vspace{-4pt}
    \caption{Proposed non-autoregressive ASR framework using CTC outputs. The model is trained with the joint CTC and mask-predict objectives. During inference, each token in the CTC outputs is replaced with the mask tokens based on the CTC confidence. The masked tokens are then fed into the decoder which predicts masks conditioning on the other unmasked tokens.}
    \label{fig:proposed_decoding}
\end{figure}

Non-autoregressive models must know the length of the output sequence
to predict the entire sequence in parallel.
For example, in the beginning of the CMLM decoding, 
the output length must be given to initialize the target sequence with the masked tokens.
To deal with this problem, 
in machine translation, 
the output length is predicted by training a fertility model~\cite{gu2017non} or 
introducing a special \texttt{<LENGTH>} token in the encoder~\cite{ghazvininejad2019mask}.
In speech recognition, however, 
due to the difference between the input acoustic signals and the output linguistic symbols, 
we experienced predicting the output length is rather challenging, 
e.g. the length of the input utterances of the same transcription vary greatly depending on the speed or the duration of silence.
% varying length of the output sequence with a small unit (i.e. characters or BPEs~\cite{sennrich2015neural}), 
% we experienced predicting the output length is rather challenging.
\cite{chen2019non} simply makes the decoder to predict the position of \texttt{<EOS>} token to deal with the output length.
However, the author analyzes that this prediction is vulnerable to the output sequence with a long length because the model is likely to make more mistakes in predicting long masked sequence and the error propagated to the later decoding degrades the recognition performance.
To compensate this problem, 
this work uses beam-search with CTC and language model to obtain the reasonable performances, 
which leads to a slow down of the overall decoding speed, 
making the advantage of non-autoregressive framework less effective.

To tackle this problem regarding the initialization of the target sequence, 
we consider using the CTC outputs as the initial sequence for decoding.
Figure~\ref{fig:proposed_decoding} shows the proposed decoding framework based on the inference of CTC. 
CTC outputs are first obtained through a single calculation of the encoder and the decoder works as to refine the CTC outputs by attending to the whole sequence.

In this work, we use ``greedy'' result of CTC, which is obtained without using prefix search~\cite{graves2006connectionist}, because it reduces the computational cost and the mistakes caused by conditional independence is expected to be corrected using the decoder.
The posterior probability of each greedy CTC result $\hat{Y} = \{ \hat{y}_l \in \beta(A) | l=1,...,L' \}$ is calculated as follows:
\begin{equation}
    \hat{P}(\hat{y}_l | X) = \max_{j} \Big( P(A_{l, j} | X) \Big),
\end{equation}
where $A_l$ is the consective same alignments that corresponds to the aggregated token $y_l$.
Then part of $\hat{Y}$ is masked-out based on a confidence based on the probability $\hat{P}$ as follows:
\begin{eqnarray}
    \hat{Y}_{\mathrm{mask}} = \{ y_l \in \hat{Y} | \hat{P}(y_l | X) < P_{\mathrm{thres}} \}
\end{eqnarray}
where $P_{\mathrm{thres}}$ is a threshold probability for deciding the target token is masked or not.
Finally, $\hat{Y}_{\mathrm{mask}}$ is predicted conditioning on the high-confident tokens $\hat{Y}_{\mathrm{obs}} = \hat{Y} \setminus \hat{Y}_{\mathrm{mask}}$ and the input sequence $X$ as in Eq. (5).

We also investigated applying one of iterative decoding methods called easy-first~\cite{goldberg2010efficient, chen2019non}.
Starting with the masked CTC output,
the masked tokens are gradually predicted by a confidence based on CMLM probability.
In the $n$-th decoding iteration, 
$\hat{y}_{l} \in \hat{Y}_{\mathrm{mask}}^{(n)}$ is updated as follows:
\begin{equation}
    \hat{y}_l= \argmax_{w} P_{\mathrm{cmlm}} (\hat{y}_l = w | Y_{\mathrm{obs}}^{(n)}, X),
\end{equation}
where position $l$, which mask to be predicted, is selected by top $C$ tokens with the highest probabilities.
By defining $C = [L / K]$, 
the number of total decoding iterations can be controlled in a constant $K$ iterations.

With this proposed non-autoregressive training and decoding, 
the model does not need to take care about predicting the output length.
Moreover, 
decoding by refining CTC outputs with the mask prediction is expected to compensate the mistakes come from the contextual independence assumption.

